Sequential Reptile: Inter-Task Gradient Alignment for Multilingual Learning

Multilingual models jointly pretrained on multiple languages have achieved remarkable performance on various multilingual downstream tasks. Moreover, models finetuned on a single monolingual downstream task have shown to generalize to unseen languages. In this paper, we first show that it is crucial for those tasks to align gradients between them in order to maximize knowledge transfer while minimizing negative transfer. Despite its importance, the existing methods for gradient alignment either have a completely different purpose, ignore inter-task alignment, or aim to solve continual learning problems in rather inefficient ways. As a result of the misaligned gradients between tasks, the model suffers from severe negative transfer in the form of catastrophic forgetting of the knowledge acquired from the pretraining. To overcome the limitations, we propose a simple yet effective method that can efficiently align gradients between tasks. Specifically, we perform each inner-optimization by sequentially sampling batches from all the tasks, followed by a Reptile outer update. Thanks to the gradients aligned between tasks by our method, the model becomes less vulnerable to negative transfer and catastrophic forgetting. We extensively validate our method on various multi-task learning and zero-shot cross-lingual transfer tasks, where our method largely outperforms all the relevant baselines we consider.

==> [ICLR 2022] Sequential Reptile/0_abstract.tex <==
\begin{abstract}
Multilingual models jointly pretrained on multiple languages have achieved remarkable performance on various multilingual downstream tasks. Moreover, models finetuned on a single monolingual downstream task have shown to generalize to unseen languages. In this paper, we first show that it is crucial for those tasks to align gradients between them in order to maximize knowledge transfer while minimizing negative transfer. Despite its importance, the existing methods for gradient alignment either have a completely different purpose, ignore inter-task alignment, or aim to solve continual learning problems in rather inefficient ways. As a result of the misaligned gradients between tasks, the model suffers from severe negative transfer in the form of catastrophic forgetting of the knowledge acquired from the pretraining. To overcome the limitations, we propose a simple yet effective method that can efficiently align gradients between tasks. Specifically, we perform each inner-optimization by sequentially sampling batches from all the tasks, followed by a Reptile outer update. Thanks to the gradients aligned between tasks by our method, the model becomes less vulnerable to negative transfer and catastrophic forgetting. We extensively validate our method on various multi-task learning and zero-shot cross-lingual transfer tasks, where our method largely outperforms all the relevant baselines we consider.
\end{abstract}


==> [ICLR 2022] Sequential Reptile/1_introduction.tex <==
\section{introduction}
Multilingual language models~\citep{bert, xlm, xlm-r, mbart, marge, mt5} have achieved impressive performance on a variety of multilingual natural language processing (NLP) tasks. Training a model with multiple languages jointly can be understood as a multi-task learning (MTL) problem where each language serves as a distinct task to be learned~\citep{grad-vac}. 
% Main point of our argument
The goal of MTL is to make use of relatedness between tasks to improve generalization without negative transfer~\citep{mtl-classic-2,mtl-classic,mtl-classic-3, wang-avoid-negative-transfer,negative-interference}. Likewise, when we train with a downstream multilingual MTL objective, we need to maximize knowledge transfer between the languages while minimizing negative transfer between them. This is achieved by developing an effective MTL strategy that can prevent the model from memorizing task-specific knowledge not easily transferable across the languages.

Such MTL problem is highly related to the gradient alignment between the tasks, especially when we finetune a well-pretrained model like multilingual BERT~\citep{bert}. 
We see from the bottom path of Fig.~\ref{fig:concept} that the cosine similarity between the task gradients (gradients of MTL losses individually computed for each task) tend to gradually decrease as we finetune the model with the MTL objective.
It means that the model gradually starts memorizing task-specific (or language-specific) knowledge not compatible across the languages, which can cause a negative transfer from one language to another. In case of finetuning the well-pretrained model, we find that it causes catastrophic forgetting of the pretrained knowledge. Since the pretrained model is the fundamental knowledge shared across all NLP tasks, such catastrophic forgetting can severely degrade the performance of all tasks. Therefore, we want our model to maximally retain the knowledge of the pretrained model by finding a good trade-off between minimizing the downstream MTL loss and maximizing the cosine similarity between the task gradients, as illustrated in the upper path of Fig.~\ref{fig:concept}. In this paper, we aim to solve this problem by developing an MTL method that can efficiently align gradients across the tasks while finetuning the pretrained model.


% limitation of pcgrad
There has been a seemingly related observation by \cite{pcgrad} that the conflict (negative cosine similarity) between task gradients makes it hard to optimize the MTL objective. They propose to manually alter the direction of task gradients whenever the task gradients conflict to each other. However, their intuition is completely different from ours. They \emph{manually} modify the task gradients whenever the gradient conflicts happen, which leads to more aggressive optimization of MTL objective. In case of finetuning a well-pretrained model, we find that it simply leads to catastrophic forgetting. Instead, we aim to make the model converge to a point where task gradients are naturally aligned, leading to less aggressive optimization of the MTL objective (See the upper path of Fig.~\ref{fig:concept}).


Then a natural question is if we can alleviate the catastrophic forgetting with early stopping. Our observation is that whereas early stopping can slightly increase cosine similarity to some extent, it is not sufficient to find a good trade-off between minimizing MTL objective and maximizing cosine similarity to improve generalization (See Fig.~\ref{fig:concept}).
It means that we may need either an implicit or explicit objective for gradient alignment between tasks. Also, \cite{recadam} recently argue that we can mitigate catastrophic forgetting by adding $\ell_2$ regularization to AdamW optimizer~\citep{adamw}. They argue that the resultant optimizer penalizes $\ell_2$ distance from the pretrained model during the finetuning stage. However, unfortunately we find that their method is not much effective in preventing catastrophic forgetting in the experimental setups we consider.

\input{concept_fig}
 
% limitation of reptile
On the other hand, Reptile~\citep{reptile} implicitly promotes gradient alignment between mini-batches \emph{within a task}. Reptile updates a shared initial parameter individually for each task, such that the task gradients are not necessarily aligned across the tasks. In continual learning area, MER~\citep{mer} and La-MAML~\citep{la-maml} propose to align the gradients between sequentially incoming tasks in order to maximally share the progress on their objectives. However, as they focus on continual learning problems, they require explicit memory buffers to store previous task examples and align gradients with them, which is complicated and costly.  Further, their methods are rather inefficient in that the inner-optimization is done with batch size set to 1, which takes significantly more time than usual batch-wise training. Therefore, their methods are not straightforwardly applicable to multilingual MTL problems we aim to solve in this paper.


In this paper, we show that when we finetune a well-pretrained model, it is sufficient to align gradients between the currently given downstream tasks in order to retain the pretrained knowledge, without accessing the data used for pretraining or memory buffers.
Specifically, during the finetuning stage, we sequentially sample mini-batches \emph{from all the downstream tasks} at hand to perform a single inner-optimization, followed by a Reptile outer update. Then, we can efficiently align the gradients between tasks based on the implicit dependencies between the inner-update steps. This procedure, which we call \emph{Sequential Reptile}, is a simple yet effective  method that can largely improve the performance of various downstream multilingual tasks by preventing negative transfer and catastrophic forgetting in an efficient manner. We summarize our contributions as follows. 

\vspace{-0.1in}
\begin{itemize}[itemsep=1mm, parsep=0pt, leftmargin=*]
    \item We show that when finetuning  a well-pretrained model, gradients not aligned between tasks can cause negative transfer and catastrophic forgetting of the knowledge acquired from the pretraining.
    
    \item To solve the problem, we propose \emph{Sequential Reptile}, a simple yet effective MTL method that  efficiently aligns gradients between tasks, thus prevents negative transfer and catastrophic forgetting. 
    
    \item We extensively validate our method on various MTL and zero-shot cross-lingual transfer tasks, including question answering, named entity recognition and natural language inference tasks, in which our method largely outperforms all the baselines.
\end{itemize}

%which enforce models to learn common knowledge among tasks and transfer it to improve generalization on MTL and zero-shot cross-lingual transfer.
%\item We empirically show that our method is effective for preventing catastrophic forgetting of linguistic knowledge from pretraining, which is crucial for finetuning a language model with MTL objective and zero-shot cross lingual transfer.
%To verify the efficacy our model, we empirically show that it significantly outperforms all the baselines on question answering and named entity recognition for MTL. Moreover, we formulate zero-shot cross-lingual transfer as MTL and show that ours achieves the best performance among the relevant baselines on QA and natural language inference task.
%To summarize, our contribution in this work is threefold:

%We exploit the implicit gradient alignments inherent in Reptile~\citep{reptile}.
%, such that the inner-products between mini-batch gradients \emph{within a task} is maximized by the update procedure. % interleave the mini-batches sampled from different tasks. %Then we sequentially perform gradient descent with the sampled batches. 
%After the pre-defined number of inner updates, we compute the meta-gradient by summing up the individual task gradients evaluated with the mini-batches. 
%Since each task gradient is dependent to the previous inner update computed from different tasks, a model is enforced to align all the task gradients involved in MTL. 
%Thanks to the gradient alignment of Sequential Reptile,  %Otherwise, task gradient conflicts to each others. In addition, the gradient alignment prevents the model to aggressively minimize MTL loss since gradients conflict to each to other on local optima. As a result the trained model is located to be close to the initial pretrained parameters, which alleviates the catastrophic forgetting.  


==> [ICLR 2022] Sequential Reptile/2_related_work.tex <==
\section{related works}
\paragraph{Multi-task Learning}
The goal of MTL is to leverage relatedness between tasks for effective knowledge transfer while preventing negative interference between them~\citep{mtl-task-relatdness, mtl-classic-2, mtl-classic-3}. GradNorm~\citep{gradnorm} tackles task imbalance problem by adaptively weighting each task loss. Another line of literature propose to search Pareto optimal solutions which represent trade-offs between the tasks~\citep{pareto-mtl, pareto-mtl-2}. Recently, ~\cite{pcgrad} and \cite{grad-vac} propose to manually resolve the conflict between task gradients to more aggressively optimize the given MTL objective. However, their goal is completely different from ours because here we focus on preventing negative transfer by finding a model that can naturally align the task gradients without such manual modifications.


\vspace{-0.1in}
\paragraph{Multilingual Language Model}
Training a multilingual language model is a typical example of multi-task learning. Most of the previous works focus on jointly pretraining a model with hundreds of languages to transfer common knowledge between the languages~\citep{bert, xlm, xlm-r, mbart, marge, mt5}. Some literature show the limitation of jointly training the model with multilingual corpora~\citep{nmt-wild,negative-interference}. Several follow-up works propose to tackle the various accompanying problems such as post-hoc alignment~\citep{post-alignment, post-alignment-2}, data balancing~\citep{balancing-nmt} and loss curvature-aware optimization to improve the performance of low resource languages~\citep{cat}. In this paper, we focus on how to finetune a well pretrained multilingual language model by preventing catastrophic forgetting of the pretrained knowledge.

\vspace{-0.1in}
\paragraph{Zero-shot Cross Lingual Transfer}
Zero-shot cross-lingual transfer is to train a model with monolingual labeled data and evaluate it on some unseen target languages without further finetuning the model on the target languages. \cite{x-maml} utilize meta-learning to learn how to transfer knowledge from high resource languages to low resource ones. 
\cite{pretraining-align} and \cite{post-pretraining-align} leverage a set of paired sentences from different languages to train the model and minimize the distance between the representation of the paired sentences.
Instead, we partition the monolingual labeled data into groups and consider them as a set of tasks for multi-task learning.


==> [ICLR 2022] Sequential Reptile/3_method.tex <==
\section{Approach}
The goal of multi-task learning (MTL) is to estimate a model parameter $\phi$ that can achieve good performance across all the given $T$ tasks, where each task $t=1,\dots,T$ has task-specific data $\mathcal{D}_t$. We learn $\phi$ by minimizing the sum of task losses.
\begin{align}
     \min_{\phi} \sum_{t=1}^T\mathcal{L}(\phi;\mathcal{D}_t) + \lambda \Omega(\phi)
\label{mtl}
\end{align}
where $\Omega(\phi)$ is a regularization term and $\lambda \geq 0$ is an associated coefficient.


\vspace{-0.1in}
\paragraph{Reptile}
We briefly review Reptile~\citep{reptile}, an efficient first-order meta-learning method suitable for large-scale learning scenario. We show that Reptile has an approximate learning objective of the form in Eq.~\ref{mtl}. Although Reptile is originally designed for learning a shared initialization, we can use the initialization $\phi$ for actual predictions without any adaptation~\citep{mer}. Firstly, given a set of $T$ tasks, we \emph{individually} perform the task-specific optimization from $\phi$. Specifically, for each task $t=1,\dots,T$, we perform the optimization by sampling mini-batches $\mathcal{B}_t^{(1)},\dots,\mathcal{B}_t^{(K)}$ from task data $\mathcal{D}_t$ and taking gradient steps with them.
\begin{equation}
\theta_t^{(0)} = \phi,\qquad \theta^{(k)}_{t} = \theta^{(k-1)}_{t} -\alpha \frac{\partial\mathcal{L}(\theta^{(k-1)}_{t}; \mathcal{B}_{t}^{(k)})}{\partial \theta^{(k-1)}_{t}}
\label{inner-reptile}
\end{equation}
for $k=1,\dots,K$, where $\alpha$ is an inner-learning rate and $\theta^{(k)}_{t}$ denotes the  task-specific parameter of task $t$ evolved from $\phi$ by taking $k$ gradient steps. After performing $K$ gradient steps for all $T$ tasks, we meta-update $\phi$ as follows:
\begin{align}
    \phi \leftarrow \phi -  \eta\cdot \frac{1}{T} \sum_{t=1}^T \text{MG}_t(\phi),\quad\text{where}\quad \text{MG}_t(\phi) = \phi -\theta^{(K)}_{t}    
\end{align}    
where $\eta$ denotes an outer-learning rate. \cite{reptile} show that expectation of $\text{MG}_t(\phi)$ over the random sampling of batches, which is the meta-gradient of task $t$ evaluated at $\phi$, can be approximated as follows based on Taylor expansion:
\begin{equation}
    \begin{gathered}
        \mathbb{E}\left[\text{MG}_t(\phi) \right] 
        \approx 
        \frac{\partial}{\partial \phi}\mathbb{E}\left[\sum_{k=1}^K  \mathcal{L} (\phi; \mathcal{B}^{(k)}_{t}) -\frac{\alpha}{2} \sum_{k=1}^K\sum_{j =1}^{k-1}\ip{\frac{\partial \mathcal{L}(\phi; \mathcal{B}^{(k)}_{t}) }{\partial\phi}}{\frac{\partial \mathcal{L}(\phi; \mathcal{B}^{(j)}_{t}) }{\partial \phi}}\right] 
        \label{eq:reptile_taylor}
    \end{gathered}
\end{equation}
where $\ip{\cdot}{\cdot}$ denotes a dot product. We can see that $\mathbb{E}[\text{MG}_t(\phi)]$ approximately minimizes the task-specific loss (first term) and maximizes the inner-products between gradients computed with different batches (second term). The inner-learning rate $\alpha$ controls the trade-off between them. However, the critical limitation is that the dot product does not consider aligning gradients computed from different tasks. This is because each inner-learning trajectory consists of the batches $\mathcal{B}_t^{(1)},\dots,\mathcal{B}_t^{(K)}$ sampled from the same task data $\mathcal{D}_t$.



\begin{figure}[t]
	\centering
	\includegraphics[width=0.85\linewidth]{figures/models.pdf}
    \vspace{-0.1in}
	\caption{\small Comparison between the methods.}
	\label{fig:models}
	\vspace{-0.25in}
\end{figure} 

\subsection{Sequential Reptile}\label{sec:seq-reptile}
In order to consider gradient alignment \emph{across tasks} as well, we propose to let the inner-learning trajectory consist of mini-batches randomly sampled \emph{from all tasks}, which we call \emph{Sequential Reptile}.

Unlike Reptile where we run $T$ task-specific inner-learning trajectory (in parallel), now we have a single learning trajectory responsible for all $T$ tasks (See Figure~\ref{fig:models}). Specifically, for each inner-step $k$, we randomly sample a task index $t_k \in \{1,\dots,T\}$ and a corresponding mini-batch $\mathcal{B}_{t_k}^{(k)}$, and then sequentially update $\theta^{(k)}$ as follows.
\begin{equation}
\begin{gathered}
    \theta^{(0)} = \phi,\qquad 
    \theta^{(k)} = \theta^{(k-1)} - \alpha \frac{\partial \mathcal{L}(\theta^{(k-1)}; \mathcal{B}_{t_k}^{(k)}) }{\partial \theta^{(k-1)} },\quad\text{where}\quad t_k \sim \text{Cat}(p_1, \ldots, p_T)
\label{inner-seq-reptile}
\end{gathered}
\end{equation}
$\text{Cat}(p_1, \ldots, p_T)$ is a categorical distribution parameterized by $p_1,\dots,p_T$, the probability of each task to be selected. For example, we can let
$p_t \propto (N_t)^{q}$ where $N_t$ is the number of training instances for task $t$ and $q$ is some constant.
After $K$ gradient steps with Eq.~\ref{inner-seq-reptile}, we update $\phi$ as follows
\begin{align}
    \phi \leftarrow \phi -\eta \cdot \text{MG}(\phi),\quad\text{where}\quad\text{MG}(\phi) = \phi - \theta^{(K)} 
\end{align}
Again, based on Taylor expansion, we have the following approximate form for expectation of the meta-gradient $\text{MG}(\phi)$ over the random sampling of tasks (See derivation in Appendix~\ref{derivation}).
\begin{equation}
    \mathbb{E}\left[\text{MG}(\phi) \right] \approx \frac{\partial}{\partial\phi}\mathbb{E}\left[\sum_{k=1}^K \mathcal{L} (\phi; \mathcal{B}^{(k)}_{t_k}) -\frac{\alpha}{2} \sum_{k=1}^K\sum_{j =1}^{k-1}\ip{\frac{\partial \mathcal{L} (\phi; \mathcal{B}^{(k)}_{t_k}) }{\partial\phi}}{\frac{\partial \mathcal{L} (\phi; \mathcal{B}^{(j)}_{t_{j}}) }{\partial \phi}}\right]
\label{seq-meta-grad}
\end{equation}
Note that the critical difference of Eq.~\ref{seq-meta-grad} from Eq.~\ref{eq:reptile_taylor} is that the dot product between the two gradients is computed from the different tasks, $t_k$ and $t_j$. Such inter-task dependency appears as we randomly sample batches from all the tasks sequentially and compose a single learning trajectory with them. As a result, Eq.~\ref{seq-meta-grad}, or Sequential Reptile promotes the gradient alignments between the tasks, preventing the model from memorizing language specific knowledge. It also means that the model can find a good trade-off between minimizing the MTL objective and inter-task gradient alignment, thereby effectively preventing catastrophic forgetting of the knowledge acquired from pretraining. 



==> [ICLR 2022] Sequential Reptile/4_experiment.tex <==
\section{Experiments}
We first verify our hypothesis with synthetic experiments. We then validate our method by solving multi-task learning (MTL) and zero-shot cross-lingual transfer tasks with large-scale real datasets.

\vspace{-0.15in}
\input{contour_plot}
\label{mtl-exp}
\paragraph{Baselines} We compare our method against the following relevant baselines.
\vspace{-0.1in}
\begin{enumerate}
[itemsep=1.0mm, parsep=0pt, leftmargin=*]
    \item \textbf{STL: } Single Task Learning (STL) model trained on each single language.
    
    \item \textbf{MTL: } Base MTL model of which objective is Eq.~\ref{mtl} without the regularizer $\Omega(\phi)$.
    
    % \item \textcolor{blue}{\textbf{Adv.~\citep{dgqa}: }} \textcolor{blue}{This model aims to learn language agnostic representation with adversarial training for regularization $\Omega(\phi)$ as well as minimize MTL loss.}
    \item \textbf{GradNorm~\citep{gradnorm}: } This model tackles task imbalance problem in MTL. It prevents the training from being dominated by a single task by adaptively weighting each task gradient.  
    
    \item \textbf{PCGrad~\citep{pcgrad}: } This model aims to optimize MTL objective more aggressively by resolving gradient conflicts. Specifically, it projects a task gradient onto the other task gradients if the inner product between them is negative.
    
    \item \textbf{GradVac~\citep{grad-vac}: } Similarly to PCGrad, this model alters the task gradients to match the empirical moving average of cosine similarity between the task gradients.
    
    \item \textbf{RecAdam~\citep{recadam}: } A model trained with RecAdam optimizer to prevent catastrophic forgetting by penalizing $\ell_2$ distance from the the pretrained model.
    
    \item \textbf{Reptile~\citep{reptile}: } A first-order meta-learning method suitable for large-scale learning scenario. Unlike our method, Reptile performs inner-optimization individually for each task.
    
    \item \textbf{Sequential Reptile: } Our method that can align gradients across the tasks by composing the inner-learning trajectory with all the tasks.
    
\end{enumerate}
\vspace{-0.1in}
\subsection{Synthetic Experiments}\label{synthetic-exp}
We first verify our hypothesis with the following synthetic experiments. We define three local optima $x_1 = (0,10), x_2 = (0,0)$, and $x_3 = (10,0)$ in a 2-dimensional space. 
Then, we define three tasks as minimizing each of the following loss functions w.r.t $\phi \in \mathbb{R}^2$.
\begin{equation*}
    \mathcal{L}_i(\phi) = -200\cdot\exp\left(0.2 \cdot \|\phi - x_i\|_2\right),\quad\text{for}\quad i=1,2,3.
\end{equation*}
MTL objective is defined as $\sum_{i=1}^3 \mathcal{L}_i(\phi)$, which we optimize from the initialization $(20,5)$.

\vspace{-0.1in}
\paragraph{Results and analysis}
Fig.~\ref{contour} shows the MTL loss surface and the learning trajectory of each method. We observe that except for Reptile and Sequential Reptile, all the other baselines converge to one of the MTL local minima, failing to find a reasonable solution that may generalize better across the tasks. While Reptile can avoid such a minimum, the resultant solution has very low cosine similarity (See Fig.~\ref{heatmap}) because it does not enforce gradient alignments between tasks. On the other hand, Figure~\ref{heatmap} shows that our Sequential Reptile tends to find a reasonable trade-off between minimizing MTL loss and maximizing cosine similarity, thanks to the implicit enforcement of inter-task gradient alignment in Eq.~\ref{seq-meta-grad}.



\input{tables/mtl_qa}
\input{tables/mtl_ner}

\subsection{Multi-Task Learning}

We next verify our method with large-scale real datasets. We consider multi-task learning tasks such as multilingual Question Answering (QA) and Named Entity Recognition (NER). For QA, we use  ``Gold passage" of   TYDI-QA~\citep{tydi} dataset where a QA model predicts a start and end position of answer from a paragraph for a given question. For NER, we use WikiAnn dataset~\citep{ner-data} where a model classifies each token of a sentence into three classes.
% --- Beginning of entity (B), Inside of entity (I), and Outside of entity (O). 
We consider each language as a distinct task and train MTL models.

\vspace{-0.05in}
\paragraph{Implementation Details} For all the experiments, we use multilingual BERT~\citep{bert} base model as a backbone network. 
We fintune it with AdamW~\citep{adamw} optimizer, setting the inner-learning rate $\alpha$ to $3\cdot 10^{-5}$. We use batch size $12$ for QA and $16$ for NER, respectively. For our method, we set the outer learning rate $\eta$ to $0.1$ and the number inner-steps $K$ to 1000. Following~\cite{grad-vac}, for all the baselines, we sample eight tasks proportional to $p_t \propto ({N_t})^{1/5}$ where $N_t$ is the number of training instances for task $t$. For our Sequential Reptile, we set the parameter of the categorical distribution in Eq.~\ref{inner-seq-reptile} to the same $p_t$. 

\vspace{-0.05in}
\paragraph{Results}
We compare our method, Sequential Reptile against the baselines on QA and NER tasks. Table~\ref{mtl-qa} shows the results of QA task. We see that our method outperforms all the baselines including STL on most of the languages. Interestingly, all the other baselines but ours underperform STL on Arabic language which contains the largest number of training instances ($2\sim 3$ times larger than the other languages. See Appendix~\ref{sec:data-stat} for more information about data statistics). It implies that the baselines suffer from negative transfer while ours is relatively less vulnerable. We can observe essentially the same tendency for NER task, which is a highly imbalanced such that the low-resource languages can have around 100 training instance, while the high-resource languages can have around 5,000 to 20,000 examples. Table~\ref{mtl-ner} shows the results of NER task. We see that all the baselines but ours highly degrade the performance on high resource languages --- de, en, es, hi, mr and tl, which means that they fail to address the imbalance problem properly and suffer from severe negative transfer. Even GradNorm is not effective in our experiments, which is developed to tackle the task imbalance problem by adaptively scaling task losses.

\input{cos_sim_all}
\input{l2_mlm_plot}

\vspace{-0.05in}
\paragraph{Analysis} We next analyze the source of performance improvements. Our hypothesis is that our method can effectively filter out language specific knowledge when solving the downstream tasks, which prevents negative transfer and helps retain linguistic knowledge acquired from the pretraining. 
\input{tables/mtl_zero_qa}

Firstly, we quantitatively measure the cosine similarity between the gradients computed from different tasks in Fig.~\ref{cos-sim-qa} (QA) and Fig.~\ref{cos-sim-ner} (NER). We see from the figure that our Sequential Reptile shows the highest cosine similarity as expected, due to the approximate learning objective in Eq.~\ref{seq-meta-grad}. Such high cosine similarity between the task gradients implies that the model has captured the common knowledge well transferable across the languages. This is in contrast to the other baselines whose task gradients can have even negative cosine similarity with high probability. Such different gradient directions mean that the current model has memorized the knowledge not quite transferable across the languages, which can cause negative transfer from one language to others.

As a result of such negative transfer, we see from Fig.~\ref{mlm-loss-seen} and Fig.~\ref{mlm-loss-unseen} that the baselines suffer from catastrophic forgetting. In those figures, high MLM losses on seen (Fig.~\ref{mlm-loss-seen}) and unseen languages (Fig.~\ref{mlm-loss-unseen}) mean that the models have forgotten how to reconstruct the masked sentences, which is the original training objective of BERT. On the other hand, our method shows relatively lower MLM loss, demonstrating its effectiveness in preventing negative transfer and thereby alleviating the catastrophic forgetting. We further confirm this tendency in Fig.~\ref{l2-dist} by measuring the $\ell_2$ distance from the initially pretrained BERT model. We see that the distance is much shorter for our method than the baselines, which implies that ours can better retain the linguistic knowledge than the baselines.

We can actually test if the finetuned models have acquired knowledge transferable across the languages by evaluating on some unseen languages without further finetuning. In Table~\ref{mtl-zero-qa}, we test the finetuned QA models on five unseen languages from MLQA dataset~\citep{mlqa}. Again, Sequential Reptile  outperforms all the baselines. The results confirm that the gradient alignment between tasks is key for obtaining common knowledge transferable across the languages. 


\vspace{-0.08in}
\subsection{Zero-shot Cross Lingual Transfer}
\vspace{-0.02in}

We next validate our method on zero-shot cross lingual transfer task, motivated from the previous results that our method can learn common knowledge well transferable across the languages. We train a model only with English annotated data and evaluate the model on target languages without further finetuning on the target datasets. To utilize the methods of MTL, we cluster the data into four groups with Gaussian mixture model. We focus on QA and natural language inference (NLI) task. 
% where, given a premise and hypothesis, a model predicts whether the premise entails the hypothesis, contradicts the hypothesis, or neither (neutral). 
For QA, we train the model on SQuAD~\citep{squad} dataset and evaluate the model on six languages from MLQA dataset~\citep{mlqa}. For NLI, we use MNLI~\citep{mnli} dataset as a source training dataset and test the model on fourteen languages from XNLI~\citep{xnli} as a target languages. 

\vspace{-0.1in}
\paragraph{Baselines} As well as the baselines from the previous experiments, we additionally include \textbf{SWEP}~\citep{swep}. It learns to perturb word embeddings and uses the perturbed input as extra training data, which is empirically shown to be robust against out-of distribution data.  

\vspace{-0.1in}
\paragraph{Implementation Detail} We finetune multilingual BERT-base model with AdamW. For QA, we use the same hyperparameter in multi-task learning experiment. For NLI, we use batch size 32 and choose the learning rate $3\cdot 10^{-5}$ or $5\cdot 10^{-5}$ with AdamW optimizer based on the performance on the validation set. For our model, we set the outer learning rate $\eta$ to $0.1$ and the number inner steps $K$ to 1000. In order to construct multiple tasks from a single dataset,  we cluster concatenation of questions and paragraphs from SQuAD or sentences from MNLI into four groups. Following \cite{bert-cluster}, we encode the paragraphs or sentences into hidden representations with pretrained multilingual BERT. Then, we reduce the dimension of hidden representations with PCA and run Gaussian mixture model to partition them into disjoint four clusters. Since the number of training instances are almost evenly distributed for each task, we sample mini-batches from all the four tasks for all the baselines and set $p_t = 1/4$ for our model.  


\input{tables/squad_zero_qa}
\input{tables/mnli_zero_xnli}


\vspace{-0.1in}
\paragraph{Results and Analysis}
The results of zero-shot cross lingual transfer show essentially the same tendency as those of multi-task learning in the previous subsection. Firstly, our model largely outperforms all the baselines for QA and NLI tasks as shown in Table~\ref{squad-zero-qa} and~\ref{mnli-zero-xnli}. To see where the performance improvements come from, we compute the average pairwise cosine similarity between the gradients computed from different tasks in Fig.~\ref{cos-sim-hom-qa} and~\ref{cos-sim-hom-nli}. Again, Sequential Reptile shows much higher similarity than the baselines, which implies that our method can effectively filter out task-specific knowledge incompatible across the languages and thereby prevent negative transfer. As a result, Fig.~\ref{mlm-loss-hom-qa} and~\ref{mlm-loss-hom-nli} show that our method can better retain the linguistic knowledge obtained from the pretraining in terms of relatively lower MLM loss. Further, Fig.~\ref{l2-dist-hom-qa} and \ref{l2-dist-hom-nli} confirm this tendency with shorter $\ell_2$ distance from the initially pretrained BERT model.




\input{l2_mlm_hom_plot}
\input{analysis_plot}

\vspace{-0.05in}
\subsection{Further Analysis}
\vspace{-0.05in}

\textbf{(a) Trade-off shown in Fig.~\ref{fig:concept}: }
In Fig.~\ref{trade-off}, MTL loss and cosine similarity decrease as we finetune the model from top-right to the bottom-left corner. Meanwhile, Sequential Reptile shows much higher cosine similarities between task gradients at the points of similar MTL losses, achieving better trade-off than Reptile. It explains why simple early stopping cannot outperform Sequential Reptile (see Fig.~\ref{efficiency}) that directly enforces gradient alignment across tasks.

\textbf{(b) Effect of the strength of gradient alignment: } 
Then the next question is, how can we further control the trade-off to maximize performance? According to Eq.~\ref{seq-meta-grad}, we can strengthen or weaken the gradient alignment by increasing or decreasing the inner-learning rate $\alpha$, respectively. Fig.~\ref{lr-cos-em} shows that while we can control the cosine similarity by varying $\alpha$ as expected, the best-performing $\alpha$ is around $3\cdot 10^{-5}$, which is indeed the most commonly used value for finetuning the BERT model.

\textbf{(c) Computational efficiency: } 
Lastly, one may suspect training Sequential Reptile takes significantly longer wall clock time because inner steps are not parallelizable as in Reptile (See Fig.~\ref{fig:models}). This is not true. Fig.~\ref{efficiency} shows that whereas base MTL requires around $40$K gradient computations to achieve 64 EM score, Sequential Reptile requires only around $15$K. As a result, although we run Sequential Reptile with a single GPU at a time, the wall-clock time becomes even comparable to the base MTL that we run in parallel with $8$ GPUs. Please see wall clock comparison on Appendix~\ref{appendix-analysis}.



==> [ICLR 2022] Sequential Reptile/5_conclusion.tex <==
\vspace{-0.05in}
\section{conclusion}
\vspace{-0.05in}
We showed that when finetuning a well-pretrained language model, it is important to align gradients between the given set of downstream tasks to prevent negative transfer and retain linguistic knowledge acquired from the pretraining. We proposed a simple yet effective method aligning gradients between tasks with efficiency. Specifically, instead of performing multiple inner-optimizations separately for each task, we performed a single inner-optimization by sequentially sampling batches from all the tasks, followed by a Reptile outer update. We extensively validated the efficacy of our method on various MTL and zero-shot cross-lingual transfer tasks, where ours largely outperformed all the baselines we considered.


\noindent
\textbf{Acknowledgements}
% AI, ERC, samsung, samsung, AI-hub, nrf, naver
This work was supported by Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government(MSIT)  (No.2019-0-00075, Artificial Intelligence Graduate School Program(KAIST)), the Engineering Research Center Program through the National Research Foundation of Korea (NRF) funded by the Korean Government MSIT (NRF-2018R1A5A1059921), Samsung Research Funding Center of Samsung Electronics (No. SRFC-IT1502-51), Samsung Electronics (IO201214-08145-01), Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government(MSIT) (No. 2021-0-02068, Artificial Intelligence Innovation Hub), the National Research Foundation of Korea (NRF) funded by the Ministry of Education (NRF-2021R1F1A1061655), and KAIST-NAVER Hypercreative AI Center.


% This work was supported by Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (No.2020-0-00153), Samsung Advanced Institute of Technology (SAIT), Samsung Electronics (IO201214-08145-01), Institute of Information \& communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT)  (No.2019-0-00075, Artificial Intelligence Graduate School Program (KAIST)), and the Engineering Research Center Program through the National Research Foundation of Korea (NRF) funded by the Korean Government MSIT (NRF-2018R1A5A1059921). 



==> [ICLR 2022] Sequential Reptile/analysis_plot.tex <==
\begin{figure*}
\centering
	\begin{subfigure}{.28\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/trade_off_plot.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\caption{\small}
		\label{trade-off}
	\end{subfigure}
	\begin{subfigure}{.28\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/lr_cos_em.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\caption{\small}
		\label{lr-cos-em}
	\end{subfigure}
	\begin{subfigure}{0.42\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/early_stop.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\caption{\small}
		\label{efficiency}
	\end{subfigure}
	\vspace{-0.15in}
	\caption[cos-sim]{\small \textbf{(a) Trade-off shown in Fig.~\ref{fig:concept}:} average cosine similarity between task gradients vs. MTL training loss. \textbf{(b) Effect of the strength of gradient alignment:} Average cosine similarity between task gradients and test performance (EM) vs. inner-learning rate. \textbf{(c) Computational efficiency:} Test performance (EM) vs. the cumulative count of (inner-) gradient steps used for training.  
	}
	\vspace{-0.1in}
	\label{further-analysis}
\end{figure*}


==> [ICLR 2022] Sequential Reptile/concept_fig.tex <==
\begin{figure}[t]
    \vspace{-0.1in}
	\centering
	\includegraphics[height=3cm]{figures/concept2.pdf}
    \vspace{-0.05in}
	\caption{\small \textbf{Concepts.} Black arrows denote finetuning processes. The darker the part of the arrows, the lower the MTL loss. Upper and bottom path shows better and worse trade-off, respectively. Colored arrows denote task gradients. Blue and red color shows high and low cosine similarity, respectively. We demonstrate this concept with the actual experimental results in Fig.~\ref{trade-off}.}
	\label{fig:concept}
 	\vspace{-0.2in}
\end{figure}

==> [ICLR 2022] Sequential Reptile/contour_plot.tex <==
\begin{figure*}
\centering
\vspace{-0.15in}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/mtl_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small MTL}
		\label{mtl-contour}
	\end{subfigure}%
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/gradnorm_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small GradNorm}
		\label{gradnorm}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/pcgrad_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small PCGrad}
		\label{pcgrad-contour}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/gradvac_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small GradVac}
		\label{gradvac-contour}
	\end{subfigure}
	
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/rec_adam_mtl_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small RecAdam}
		\label{recadam-contour}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/reptile_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small Reptile}
		\label{reptile-contour}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/reptile_sequence_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small Seq.Reptile}
		\label{seq-reptile-contour}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/heat_map.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small Cos. sim. btw task gradients.}
		\label{heatmap}
	\end{subfigure}
	\vspace{-0.1in}
	\caption[contour]{\small \textbf{(a)}$\sim$\textbf{(g)} Loss surface and learning trajectory of each method. \textbf{(h)} 
	Heatmap shows average pair-wise cosine similarity between the task gradients.
	}
	\vspace{-0.17in}
	\label{contour}
\end{figure*}

==> [ICLR 2022] Sequential Reptile/contour_plot_2.tex <==
\begin{figure*}
\centering
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_2/mtl_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{mtl-contour-2}
	\end{subfigure}%
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_2/gradnorm_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{gradnorm-2}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_2/pcgrad_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{pcgrad-contour-2}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_2/gradvac_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{gradvac-contour-2}
	\end{subfigure}
	
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_2/rec_adam_mtl_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{recadam-contour-2}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_2/reptile_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{reptile-contour-2}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_2/reptile_sequence_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{seq-reptile-contour-2}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_2/heat_map.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{heatmap-2}
	\end{subfigure}
	\vspace{-0.2in}
	\caption[contour]{
	}
	\label{contour-2}
\end{figure*}

==> [ICLR 2022] Sequential Reptile/contour_plot_3.tex <==
\begin{figure*}
\vspace{-0.25in}
\centering
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_3/mtl_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{mtl-contour-3}
	\end{subfigure}%
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_3/gradnorm_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{gradnorm-3}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_3/pcgrad_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{pcgrad-contour-3}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_3/gradvac_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{gradvac-contour-3}
	\end{subfigure}
	
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_3/rec_adam_mtl_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{recadam-contour-3}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_3/reptile_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{reptile-contour-3}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_3/reptile_sequence_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{seq-reptile-contour-3}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_3/heat_map.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\label{heatmap-3}
	\end{subfigure}
	\vspace{-0.1in}
	\caption[contour]{
	}
	\vspace{-0.2in}
	\label{contour-3}
\end{figure*}

==> [ICLR 2022] Sequential Reptile/contour_plot_4.tex <==
\begin{figure*}
\centering
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_4/mtl_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small}
		\label{mtl-contour-4}
	\end{subfigure}%
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_4/gradnorm_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
        \caption{\small}
		\label{gradnorm-4}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_4/pcgrad_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small}
		\label{pcgrad-contour-4}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_4/gradvac_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
        \caption{\small}
		\label{gradvac-contour-4}
	\end{subfigure}
	
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_4/rec_adam_mtl_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small}
		\label{recadam-contour-4}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_4/reptile_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small}
		\label{reptile-contour-4}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_4/reptile_sequence_losses.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.22in}
		\caption{\small}
		\label{seq-reptile-contour-4}
	\end{subfigure}
	\begin{subfigure}{0.22\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/contour_4/heat_map.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small}
		\label{heatmap-4}
	\end{subfigure}
	\vspace{-0.1in}
	\caption[contour]{\small \textbf{(a)}$\sim$\textbf{(g)} Loss surface and learning trajectory of each method. \textbf{(h)} 
	Heatmap shows average pair-wise cosine similarity between the task gradients.
	}
	\vspace{-0.1in}
	\label{contour-4}
\end{figure*}

==> [ICLR 2022] Sequential Reptile/cos_sim_all.tex <==
\begin{figure*}[t]
\centering
	\begin{subfigure}{.245\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/cos_sim_qa.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small TYDI-QA}
		\label{cos-sim-qa}
	\end{subfigure}%
	\begin{subfigure}{.245\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/cos_sim_ner.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small NER}
		\label{cos-sim-ner}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/cos_sim_qa_hom.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small SQuAD}
		\label{cos-sim-hom-qa}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/cos_sim_nli_hom.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small XNLI}
		\label{cos-sim-hom-nli}
	\end{subfigure}
	
	\vspace{-0.12in}
	\caption[cos-sim]{\small Average pair-wise cosine similarity between the gradients computed from different tasks.
	}
	\vspace{-0.15in}
	\label{cos-sim}
\end{figure*}

==> [ICLR 2022] Sequential Reptile/cos_sim_hom_nli.tex <==
\begin{wrapfigure}{o}{0.35\textwidth}
  \includegraphics[width=\linewidth]{figures/cos_sim_nli_hom.pdf}
  \vspace{-0.25in}
  \captionof{figure}{\small Avg. cos. sim. of gradients for NLI model.}
  \label{cos-sim-hom-nli}
  \vspace{-0.2in}
\end{wrapfigure}

==> [ICLR 2022] Sequential Reptile/cos_sim_hom_qa.tex <==
\begin{wrapfigure}{R}{0.29\textwidth}
\vspace{-0.2in}
  \includegraphics[width=\linewidth]{figures/cos_sim_qa_hom.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Avg. cos. sim. between QA task gradients}
  \label{cos-sim-hom-qa}
  \smallskip\par
  \includegraphics[width=\linewidth]{figures/cos_sim_nli_hom.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Avg. cos. sim. between NLI task gradients.}
  \label{cos-sim-hom-nli}
  \vspace{-0.25in}
\end{wrapfigure}



% \begin{wrapfigure}{o}{0.35\textwidth}
%   \includegraphics[width=\linewidth]{figures/cos_sim_qa_hom.pdf}
%   \vspace{-0.25in}
%   \captionof{figure}{\small Avg. cos. sim. of gradients for QA model.}
%   \label{cos-sim-hom-qa}
%   \vspace{-0.15in}
% \end{wrapfigure}



==> [ICLR 2022] Sequential Reptile/cos_sim_plot_ner.tex <==

\begin{wrapfigure}{o}{0.27\textwidth}
  \includegraphics[width=\linewidth]{figures/cos_sim_ner.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Average cosine similarity between NER task gradients.}
  \label{cos-sim-ner}
  \vspace{-0.1in}
\end{wrapfigure}


==> [ICLR 2022] Sequential Reptile/cos_sim_plot_qa.tex <==
\begin{wrapfigure}{R}{0.27\textwidth}
\vspace{-0.1in}
  \includegraphics[width=\linewidth]{figures/cos_sim_qa.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Avg. cos. sim. between QA task gradients.}
  \label{cos-sim-qa}
  \smallskip\par
  \includegraphics[width=\linewidth]{figures/cos_sim_ner.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Avg. cos. sim. between NER task gradients.}
  \label{cos-sim-ner}
  \vspace{-0.1in}
\end{wrapfigure}


% \begin{wrapfigure}{o}{0.27\textwidth}
% \vspace{-0.2in}
%   \includegraphics[width=\linewidth]{figures/cos_sim_qa.pdf}
%   \vspace{-0.3in}
%   \captionof{figure}{\small Average cosine similarity between QA task gradients.}
%   \label{cos-sim-qa}
%   \vspace{-0.1in}
% \end{wrapfigure}

==> [ICLR 2022] Sequential Reptile/l2_mlm_hom_plot.tex <==

\begin{figure*}
\centering
	\begin{subfigure}{.245\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/mlm_loss_hom_qa.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small QA }
		\label{mlm-loss-hom-qa}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/mlm_loss_hom_nli.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small NLI }
		\label{mlm-loss-hom-nli}
	\end{subfigure}
	\begin{subfigure}{.245\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/l2_dist_hom_qa.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small QA }
		\label{l2-dist-hom-qa}
	\end{subfigure}%
	\begin{subfigure}{.245\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/l2_dist_hom_xnli.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.2in}
		\caption{\small NLI }
		\label{l2-dist-hom-nli}
	\end{subfigure}
	
	\vspace{-0.1in}
	\caption[l2-mlm-hom]{\small \textbf{(a,b)} Masked Language Modeling (MLM) loss. \textbf{(c,d)} $\ell_2$ distance from the pretrained BERT model.
	}
	\vspace{-0.1in}
	\label{l2-mlm-hom}
\end{figure*}

==> [ICLR 2022] Sequential Reptile/l2_mlm_plot.tex <==
\begin{figure*}
\centering
	\begin{subfigure}{.33\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/mlm_loss_seen.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.25in}
		\caption{\small}
		\label{mlm-loss-seen}
	\end{subfigure}
	\begin{subfigure}{.32\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/mlm_loss_unseen.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.25in}
		\caption{\small}
		\label{mlm-loss-unseen}
	\end{subfigure}
	\begin{subfigure}{.33\textwidth}
		\centering
		\includegraphics[width=\linewidth]{figures/l2_dist.pdf}
		\captionsetup{justification=centering,margin=0.5cm}
		\vspace{-0.25in}
		\caption{\small}
		\label{l2-dist}
	\end{subfigure}
	\vspace{-0.1in}
	\caption[l2-mlm]{\small
	\textbf{(a, b)} Average MLM loss on \textbf{(a)} seen and \textbf{(b)} unseen languages from Common Crawl dataset. We mask $15\%$ tokens of sentences from Common Crawl dataset, which is preprocessed and provided by~\cite{ccnet}, and compute the masked language modeling loss (MLM), which is reconstruction loss of the masked sentences.
	\textbf{(c)} $\ell_2$ distance between the finetuned models and the initially pretrained BERT. 
	}
	\vspace{-0.18in}
	\label{l2-mlm}
\end{figure*}

==> [ICLR 2022] Sequential Reptile/lr_cos_plot.tex <==
\begin{wrapfigure}{R}{0.27\textwidth}
\vspace{-0.2in}
  \includegraphics[width=\linewidth]{figures/lr_cos_em.pdf}
  \vspace{-0.25in}
  \captionof{figure}{\small Plot of cos. sim. of QA task gradients and EM as a function of LR.}
  \label{lr-cos-em}
  \vspace{-0.15in}
\end{wrapfigure}


==> [ICLR 2022] Sequential Reptile/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> [ICLR 2022] Sequential Reptile/tables/glue.tex <==
\begin{table}[t]
	\small
	\centering
	\caption{\small We train MTL models on 8 tasks from GLUE dataset and report their performance.}
	\vspace{-0.1in}
	\resizebox{0.99\textwidth}{!}{
	\begin{tabular}{lccccccccc}
		\midrule[0.8pt]
		\multicolumn{10}{c}{\textbf{GLUE}} \\ 
		\midrule[0.8pt]
		{\textbf{Method}} & \textbf{CoLA}	&\textbf{MNLI}	&\textbf{MRPC}	&\textbf{QNLI}	&\textbf{QQP}	&\textbf{RTE}	&\textbf{SST2}	&\textbf{STSB}	&\textbf{Avg.} \\
		\midrule[0.8pt]

		\textbf{MTL} & {80.82}	&\textbf{83.47}	& {82.10}	&\textbf{90.50}	& {90.16}	& {68.23}	& {90.13}	&\textbf{89.73}	& {84.39}\\

		\textbf{RecAdam} & 	{81.78}	&{82.88}	&{79.16}	&{90.00}	&\textbf{90.35}	&{71.84}	&{91.20}	&{89.12}	&{84.54} \\
		\textbf{Reptile} & {82.07}	&{78.81}	&{81.30}	&{89.29}	&{87.57}	&{72.56}	&{88.76}	&{88.55}	&{83.61}\\
		\midrule[0.5pt]
		\textbf{Seq. Reptile} &\textbf{82.35}	&{83.02}	&\textbf{83.30}	&\textbf{90.50}	& {89.40}	&\textbf{73.28}	&\textbf{92.31}	&89.40	&\textbf{85.44} \\
		\bottomrule[0.8pt]
	\end{tabular}
	}
	\label{glue-mtl}
\end{table}

==> [ICLR 2022] Sequential Reptile/tables/image_classification.tex <==
% \begin{wraptable}{t}{0.3\textwidth}
% \small
% \centering
% \vskip -0.15in
% \caption{\small Average Accuracy.}
% \vspace{-0.1in}
% \resizebox{0.3\textwidth}{!}{
%     \renewcommand{\arraystretch}{0.9}
%     \begin{tabular}{lc}
%     \toprule
%     \textbf{Method}       & \textbf{Avg. Acc.}  \\
%     \midrule
%     MTL & 56.92 \\
%     Reptile & 20.96 \\
%     \midrule
%     \textbf{Seq. Reptile} & \textbf{59.74}	   \\
%     \bottomrule
% \end{tabular}
% }
% \vskip -0.1in
% \label{image-classification}
% \end{wraptable}


\begin{table}[t]
    \centering
    \caption{\small We finetune MTL models with pretrained ResNet18 backbone on 8 image classification tasks.}
    \vspace{-0.1in}
    \resizebox{0.99\textwidth}{!}{
    \begin{tabular}{lccccccccc}
    \toprule
	\multicolumn{10}{c}{\textbf{Image Classification}} \\ 
    \midrule[0.8pt]
    \textbf{Method}	&\textbf{TIN-1}	&\textbf{TIN-2}	&\textbf{CIFAR100}	&\textbf{Dogs}	&\textbf{Aircraft}	&\textbf{CUB}	
    &\textbf{F-MNIST}	&\textbf{SVHN}	&\textbf{Avg.} \\
	\midrule[0.8pt]
    \textbf{MTL}	&{56.26}	&{53.40}	&{54.43}	&{33.44}	&{44.97}	&{29.48}	&\textbf{90.10}	&{87.70}	&{56.22} \\
    \textbf{Reptile}	&{23.56}	&{23.28}	&{9.64}	&{12.20}	&{10.02}	&{6.61}	&{60.87}	&{20.86}	&{20.88} \\
    \midrule[0.8pt]
    
    \textbf{Seq. Reptile} &\textbf{58.12}	&\textbf{56.83}	&\textbf{57.46}	&\textbf{38.05}	&\textbf{59.55}	&\textbf{35.96}	&{87.44}	&\textbf{88.86}	&\textbf{60.28}\\
    \bottomrule
    \end{tabular}
    }
    \label{image-classification}
\end{table}




==> [ICLR 2022] Sequential Reptile/tables/mnli_zero_xnli.tex <==
\begin{table}[t]
	\small
	\centering
	\caption{\small Zero shot cross lingual transfer from English (MNLI) to fourteen unseen languages (XNLI).}
	\vspace{-0.15in}
	\resizebox{0.99\textwidth}{!}{
	\begin{tabular}{lccccccccccccccc}
		\midrule[0.8pt]
		\multicolumn{15}{c}{\textbf{MNLI} $\rightarrow$ \textbf{XNLI} (Accuracy)} \\ 
		\midrule[0.8pt]
		{\textbf{Method}} & \textbf{ar} & \textbf{bg} & \textbf{de} & \textbf{el} & {\textbf{es}} & \textbf{fr} & {\textbf{hi}} & \textbf{ru}& \textbf{sw} &  \textbf{th} & \textbf{tr} & \textbf{ur} & {\textbf{vi}} & {\textbf{zh}} & {\textbf{Avg.}} \\
		\midrule[0.8pt]
% 		\textcolor{blue}{\textbf{STL}} & \textcolor{blue}{65.6} & \textcolor{blue}{68.5} & \textcolor{blue}{70.9} & \textcolor{blue}{66.6} & \textcolor{blue}{73.9} & \textcolor{blue}{\textbf{74.7}} & \textcolor{blue}{59.8} & \textcolor{blue}{68.7} & \textcolor{blue}{48.8} & \textcolor{blue}{52.7} & \textcolor{blue}{60.8} & \textcolor{blue}{58.2} & \textcolor{blue}{\textbf{70.9}} & \textcolor{blue}{69.0} & \textcolor{blue}{64.9}\\
		\textbf{MTL} &{65.1}	&{68.8}	&{71.3}	&{66.4}	&{74.3}	&{72.6}	&{59.2}	&{68.8}	&{50.1}	&{52.8}	&{61.8}	&{57.9}	&{69.4}	&{69.0}	& {64.8}\\
% 		\textcolor{blue}{\textbf{Adv.}} &\textcolor{blue}{63.1}	&\textcolor{blue}{66.7}	&\textcolor{blue}{69.1}	&\textcolor{blue}{64.4}	&\textcolor{blue}{73.3}	&\textcolor{blue}{71.7}	&\textcolor{blue}{58.6}	&\textcolor{blue}{67.2}	&\textcolor{blue}{47.4}	&\textcolor{blue}{49.9}	&\textcolor{blue}{57.8}	&\textcolor{blue}{56.4}	&\textcolor{blue}{68.7}	&\textcolor{blue}{67.4}	&\textcolor{blue}{62.9} \\
		
		\textbf{RecAdam} &{63.5}	&{66.9}	&{69.4}	&{65.2}	&{72.7}	&{72.2}	&{58.8}	&{67.3}	&{49.9}	&{51.9}	&{61.0}	&{56.5}	&{67.9}	&{67.7}	&{63.6} \\
		
		\textbf{GradNorm} & {64.0}	&{68.2}	&{70.6}	&{67.0}	&{74.1}	&{72.9}	&{58.8}	&{68.0}	&{48.9}	&{53.2}	&{61.0}	&{56.8}	&{70.3}	&{69.3} & {64.5} \\
		\textbf{PCGrad} & {64.0} & {68.7} & {69.8} & {66.5} & {74.3} & {71.8} & {59.4} & {68.3} & {51.0} & {53.1} & {60.7} & {57.4} & {69.7} & {69.3} & {64.5} \\
		\textbf{GradVac} & 62.3	&67.8	&69.2	&65.9	&72.6	&72.2	&59.6	&67.1	&51.1	&52.9	&61.7	&56.4	&68.8	&68.0	&63.9 \\
		\textbf{SWEP}  & 64.8	&\textbf{69.4}	&70.5	&67.1	&74.8&	{74.4}	&58.7	&\textbf{69.7}	&49.2	&53.7	&60.2	&57.1	&69.8	&68.4	&64.8 \\
		\textbf{Reptile} & 63.3 & 66.6 & 69.4 &64.9 & 72.6 & 71.3 & 58.3 & 66.9 & 46.4 & 47.5 & 58.6 & 55.9 & 68.6 & 66.9 & 62.6 \\
		\midrule
		\textbf{Seq.Reptile}& \textbf{67.2}&	69.3&	\textbf{71.9}&	\textbf{67.8}&	\textbf{75.1}&	74.1&	\textbf{60.6}&	69.5&	\textbf{51.2}&	\textbf{55.1}&	\textbf{63.8}&	\textbf{59.1}&	{70.8}&	\textbf{69.6}&	\textbf{66.0} \\
		\bottomrule[0.8pt]
	\end{tabular}
	}
	\label{mnli-zero-xnli}
\end{table}



==> [ICLR 2022] Sequential Reptile/tables/mtl_ner.tex <==
\begin{table}[ht]
	\small
	\centering
	\caption{\small F1 score on WikiAnn dataset for NER. The best result for multilingual models is marked with bold while the underline denotes the best result among all the models including the monolingual model.}
	\vspace{-0.1in}
	\resizebox{0.99\textwidth}{!}{
	\begin{tabular}{lccccccccccccc}
		\midrule[0.8pt]
		\multicolumn{14}{c}{\textbf{Named Entity Recognition} (F1)} \\ 
		\midrule[0.8pt]
		{\textbf{Method}} & \textbf{de} & {\textbf{en}} & {\textbf{es}} & {\textbf{hi}} & {\textbf{jv}} & {\textbf{kk}} & {\textbf{mr}} & \textbf{my} & \textbf{sw} & \textbf{te}   & \textbf{tl} & \textbf{yo} & \textbf{Avg.}\\
		\midrule[0.8pt]
		\textbf{STL} & \underline{90.3} & \underline{85.0} & \underline{92.0} & \underline{89.7} & {59.1} & {88.5} & \underline{89.4} & {61.7} & {90.7} & {80.1} & \underline{96.3} & {77.7} & {83.3}\\
		\midrule
		\textbf{MTL} & {83.4} & {77.8} & {87.6} & {82.3} & {77.7} & {87.5} & {82.2} & {75.7} & {87.5} & {78.8} & {83.5} & {90.8} & {82.9}\\
% 		\textcolor{blue}{\textbf{Adv.}} & \textcolor{blue}{83.9}	& \textcolor{blue}{78.4}	& \textcolor{blue}{87.5}	& \textcolor{blue}{82.9}	& \textcolor{blue}{78.1}	& \textcolor{blue}{87.8}	& \textcolor{blue}{82.7}	& \textcolor{blue}{75.6}	& \textcolor{blue}{87.9}	& \textcolor{blue}{79.1}	& \textcolor{blue}{83.7}	& \textcolor{blue}{91.2}	& \textcolor{blue}{83.2}\\
		\textbf{RecAdam} & {84.5} & {80.0} & {88.5} & {82.7} & 
		\underline{\textbf{85.3}} & {88.5} &{84.4} & {70.3} & {89.0} & {81.6} & {87.7} & {91.6} &{84.5} \\
		
		\textbf{GradNorm} & {83.6}	&{77.5}	&{87.3}	&{82.8}	&{78.3}	&{87.8}	&{81.3}	&{73.5}	&{85.4}	&{78.9}	&{83.6}	&{91.4}	&{82.6}
		\\
		\textbf{PCGrad}  & {83.8} & {78.5} & {88.1} & {81.7} & {79.7} & {87.8} & {81.7} & {74.4} & {85.9} & {78.4} & {85.7} & {92.3} & {83.1}\\
		\textbf{GradVac}  & {83.9} & {79.5} &{88.3} & {81.8} & {80.6} & {87.5} & {82.2} & {73.9} & {87.9} & {79.4} & {87.9} & \underline{\textbf{93.0}} & {83.8}\\
		\textbf{Reptile} &{85.9}	&{82.4}	&{90.0}	&{86.3}	&{81.3}	&{81.4}	&{86.8}	&{61.8}	&{90.6}	&{72.7}	&{92.8}	& \underline{\textbf{93.0}}	&{83.7}\\
		\midrule[0.5pt]
		\textbf{Seq.Reptile} & \textbf{87.4} & \textbf{83.9} & \textbf{90.8} & \textbf{88.1} & {{85.2}} & \underline{\textbf{89.4}} & \textbf{88.9} & \underline{\textbf{76.0}} & \underline{\textbf{91.5}} & \underline{\textbf{82.5}} & \textbf{94.7} & {92.5} & \underline{\textbf{87.5}}\\
		\bottomrule[0.8pt]
	\end{tabular}
	}
	
	\label{mtl-ner}
\vspace{-0.1in}
\end{table}

==> [ICLR 2022] Sequential Reptile/tables/mtl_qa.tex <==
\begin{table}[ht]
	\small
	\vspace{-0.1in}
	\centering
	\caption{\small F1 and EM score on the TYDI-QA dataset for QA. The best result for multilingual models is marked with bold while the underline denotes the best result among all the models including the monolingual model.}
	\vspace{-0.1in}
	\resizebox{0.99\textwidth}{!}{
	\begin{tabular}{lcccccccccc}
		\midrule[0.8pt]
		\multicolumn{11}{c}{\textbf{Question Answering} (F1/EM)} \\ 
		\midrule[0.8pt]
		{\textbf{Method}} & \textbf{ar} & {\textbf{bn}} & {\textbf{en}} & {\textbf{fi}} & {\textbf{id}} & {\textbf{ko}} & {\textbf{ru}} & \textbf{sw} & \textbf{te}   & \textbf{Avg.}\\
		\midrule[0.8pt]
		\textbf{STL} & {80.5 / 65.9} & {70.9 / 58.4} & {72.0 / 59.2}  & {76.2 / 63.7} & {82.7 / 70.6} & {61.0 / 50.8} & {73.4 / 56.5} & {78.4 / 70.1} & {81.1 / 66.4} & {75.1 / 62.4}  \\
		\midrule[0.5pt]
		
		\textbf{MTL} & {79.7 / 64.7} & {{74.7} / {64.0}} & {72.8 / 61.1} & {77.8 / 64.7} & {82.9 / 71.3} & {64.0 / 53.4} & {73.9 / 57.1} &{80.5 / 72.5} & {82.5 / 67.9} & {76.5 / 64.1}\\
		
% 		\textcolor{blue}{\textbf{Adv.}} &\textcolor{blue}{80.1 / 64.8}	&\textcolor{blue}{74.82 / 64.2 }	&\textcolor{blue}{73.1 / 62.1}	&\textcolor{blue}{78.1 / 65.2 }	&\textcolor{blue}{82.8 / 72.3}	&\textcolor{blue}{65.1 / 54.4}	&\textcolor{blue}{74.3 / 57.2}	&\textcolor{blue}{80.68 / 73.4}	&\textcolor{blue}{82.53/ 68.2}	&\textcolor{blue}{76.8 / 64.5}\\
		\textbf{RecAdam} & {79.0 / 63.7} & {72.5 / 62.4} & {73.5 / 62.8}  & {76.9 / 64.9} & {82.1 / 72.2} & {64.6 / 54.5} & {73.9 / 57.6} & {80.4 / 72.9} & {82.8 / 68.4} & {76.2 / 64.4}\\ 
		
		\textbf{GradNorm} & {78.8 / 62.9} & {72.5 / 61.9} & {73.4 / 60.6} & {78.5 / 65.8} & {83.7 / 74.3} & {66.2 / 53.9} & {74.5 / 57.7} & {80.7 / 72.7} & {\underline{\textbf{83.3}} / \underline{\textbf{68.9}}} & {76.8 / 64.3} \\ 
		
		\textbf{PCGrad} & {79.9 / 65.0} & {72.6 / 61.5} & {74.6 / 62.3} & {78.3 / 65.7} & {82.7 / 73.0} & {65.9 / 56.1} & {74.2 / 57.3} & {80.6 / 73.0} & {82.5 / 68.1} & {76.8 / 64.7} \\
		
		\textbf{GradVac} & {80.1 / 64.7} & {71.5 / 59.2} & {73.0 / 61.2} & {78.6 / 65.5} & {83.1 / 72.4} & {63.8 / 53.4} & {74.1 / 57.6} & {80.6 / 72.6} & {82.2 / 67.5} & {76.3 / 63.8} \\
		
		\textbf{Reptile} & {79.8 / 65.2} & {\underline{\textbf{75.1}} / \underline{\textbf{64.1}}} & {74.0 / 62.8} & {78.8 / 65.3} & {83.8 / 73.6} & {65.7 / 55.9} & {75.5 / 58.7} & {81.4 / 72.9} & {{83.1} / 68.5} & {77.5 / 65.2} \\
		\midrule[0.5pt]
		\textbf{Seq.Reptile} & \textbf{\underline{81.2} / \underline{66.7}} & {73.9 / 62.6} & \textbf{\underline{76.7} / \underline{65.2}} & \textbf{\underline{79.4} / \underline{66.3}} & \textbf{\underline{84.9} / \underline{74.7}} & \textbf{\underline{68.0} / \underline{58.2}} & \textbf{\underline{76.8} / \underline{59.2}} & \textbf{\underline{82.9} / \underline{74.8}} & {{83.0} / {68.6}} & \textbf{\underline{78.5} / \underline{66.3}} \\
		\bottomrule[0.8pt]
	\end{tabular}
	}
	\label{mtl-qa}
\vspace{-0.05in}
\end{table}

==> [ICLR 2022] Sequential Reptile/tables/mtl_zero_qa.tex <==
\begin{table}[H]
	\small
	\centering
	\caption{\small We evaluate the model, trained with TYDI-QA dataset, on five unseen languages from MLQA dataset.}
	\vspace{-0.1in}
	\begin{tabular}{lcccccc}
		\midrule[0.8pt]
		\multicolumn{7}{c}{\textbf{TYDI-QA} $\rightarrow$ \textbf{MLQA} (F1/EM)} \\ 
		\midrule[0.8pt]
		{\textbf{Method}} & \textbf{de} & {\textbf{es}} & {\textbf{hi}} & {\textbf{vi}} & {\textbf{zh}} & {\textbf{Avg.}} \\
		\midrule[0.8pt]
		\textbf{MTL} & {50.6 / 35.8} & {54.3 / 35.4} & {45.0 / 31.2} & {53.7 / 34.8} & {52.5 / 32.0}  & {51.2 / 33.8}\\
% 		\textcolor{blue}{\textbf{Adv.}} &\textcolor{blue}{51.8 / 36.3} & \textcolor{blue}{54.5 / 36.4} &\textcolor{blue}{45.4 / 32.1} & \textcolor{blue}{54.8 / 35.1} & \textcolor{blue}{53.4 / 32.3} & \textcolor{blue}{51.9 / 34.4}\\
		\textbf{RecAdam} & {49.5 / 36.1} & {52.8 / 35.6} & {41.7 / 29.0} & {52.2 / 34.6} & {49.8 / 29.9} & {49.2 / 33.0}  \\
		
		\textbf{GradNorm} & {51.7 / 36.6} & {54.9 / 36.3} & {44.4 / 30.4} & {55.3 / 37.1} & {52.9 / 32.2} & {51.8 / 34.5}\\
		\textbf{PCGrad} & {50.6 / 36.5} & {54.5 / 36.2} & {44.1 / 31.2} & {54.4 / 34.8} & {52.4 / 31.5} & {51.1 / 34.2} \\
		\textbf{GradVac} & {50.0 / 35.4} & {53.0 / 35.2} & {41.6 / 28.6} & {52.9 / 34.9} & {51.3 / 31.2} & {49.8 / 33.1}  \\
		\textbf{Reptile} & {52.2 / 38.2} & {56.1 / 38.0}   & {45.9 / 32.1} & {56.9 / 38.2} & {53.9 / 33.2} & {53.0 / 35.9}\\
		\midrule[0.5pt]
		\textbf{Seq.Reptile} & \textbf{53.7 / 38.5} & \textbf{57.6 / 38.9} & \textbf{47.7 / 33.7} & \textbf{58.1 / 39.2} & \textbf{55.1 / 34.7} & \textbf{54.4 / 37.0} \\
		\bottomrule[0.8pt]
	\end{tabular}
	\label{mtl-zero-qa}
\end{table}
\vspace{-0.15in}

==> [ICLR 2022] Sequential Reptile/tables/squad_zero_qa.tex <==
\begin{table}
	\small
	\vspace{-0.1in}
	\centering
	\caption{\small Zero-shot cross lingual transfer from English (SQuAD) to six unseen languages (MLQA).}
	\vspace{-0.15in}
	\resizebox{0.99\textwidth}{!}{
	\begin{tabular}{lccccccc}
		\midrule[0.8pt]
		\multicolumn{8}{c}{\textbf{SQuAD} $\rightarrow$ \textbf{MLQA} (F1/EM)} \\ 
		\midrule[0.8pt]
		{\textbf{Method}} & \textbf{ar} & \textbf{de} & {\textbf{es}} & {\textbf{hi}} & {\textbf{vi}} & {\textbf{zh}} & {\textbf{Avg.}} \\
		\midrule[0.8pt]
% 		\textcolor{blue}{\textbf{STL}} & \textcolor{blue}{45.7 / 29.8} & \textcolor{blue}{57.9 / 44.3} & \textcolor{blue}{64.3 / 46.6} & \textcolor{blue}{43.8 / 29.7} & \textcolor{blue}{57.1 / 38.6} & \textcolor{blue}{\textbf{57.5} / \textbf{37.3}} & \textcolor{blue}{53.3 / 37.7}\\
		\textbf{MTL} & {48.0 / 29.9} & {59.1 / 44.6} & {64.2 / 46.2} & {44.6 / 29.0} & {56.8 / 37.8}  & {{55.2} / {34.7}} & {54.6 / 37.0}  \\
% 		\textcolor{blue}{\textbf{Adv.}} &\textcolor{blue}{47.2 / 29.4}&\textcolor{blue}{58.4 / 44.2} &\textcolor{blue}{64.3 / 46.4} &\textcolor{blue}{44.2 / 29.0}&\textcolor{blue}{56.4 / 37.3} &\textcolor{blue}{53.8 / 33.8} &\textcolor{blue}{54.0 / 36.6}\\
		\textbf{RecAdam} &{47.3 / 29.8} & {58.8 / 44.0} & {64.3 / 46.2} &{45.5 / 29.9} & {57.9 / 38.4} & {54.8 / 34.1} & {54.7 / 37.0}  \\
		
		\textbf{GradNorm} & {48.7 / 31.3} & {59.8 / 44.6} & {64.8 / 46.3} & {47.2 / 31.2} & {57.2 / 37.8} & {55.0 / 33.9} & {55.4 / 37.5}\\
		
		\textbf{PCGrad} & {47.7 / 29.8} & {59.2 / 44.1} & {65.4 / 46.1} & {41.0 / 26.0} & {57.4 / 37.4} & {54.6 / 34.0} & {54.4 / 36.2} \\
		
		\textbf{GradVac} & {45.3 / 28.3} & {58.2 / 43.4} & {63.9 / 45.9} & {42.4 / 27.9} & {56.3 / 37.1} & {53.0 / 32.9} & {53.1 / 35.9} \\
		
		\textbf{SWEP} & {49.5 / 31.0} & {60.5 / \textbf{46.2}} & {65.0 / 47.3} & {47.6 / 31.9} & {57.9 / 38.8} & {56.9 / 36.3} & {56.2 / 38.5}  \\
		
		\textbf{Reptile} & {46.8 / 29.9} & {58.7 / 44.4} & {65.1 / 47.5} & {41.5 / 27.9} & {56.1 / 37.7} & {53.9 / 33.9} & {53.6 / 36.8} \\
		\midrule[0.5pt]
		\textbf{Seq.Reptile} & \textbf{52.8} {/ \textbf{34.3}} & {\textbf{60.7} / 45.9} & \textbf{67.1 / 48.7} & \textbf{50.6 / 35.6} & \textbf{60.7 / 40.8} & {57.3 / 36.5} & \textbf{58.2 / 39.3} \\
		\bottomrule[0.8pt]
	\end{tabular}
	}
	\label{squad-zero-qa}
\end{table}

==> cos_sim_hom_nli.tex <==
\begin{wrapfigure}{o}{0.35\textwidth}
  \includegraphics[width=\linewidth]{figures/cos_sim_nli_hom.pdf}
  \vspace{-0.25in}
  \captionof{figure}{\small Avg. cos. sim. of gradients for NLI model.}
  \label{cos-sim-hom-nli}
  \vspace{-0.2in}
\end{wrapfigure}

==> cos_sim_hom_qa.tex <==
\begin{wrapfigure}{R}{0.29\textwidth}
\vspace{-0.2in}
  \includegraphics[width=\linewidth]{figures/cos_sim_qa_hom.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Avg. cos. sim. between QA task gradients}
  \label{cos-sim-hom-qa}
  \smallskip\par
  \includegraphics[width=\linewidth]{figures/cos_sim_nli_hom.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Avg. cos. sim. between NLI task gradients.}
  \label{cos-sim-hom-nli}
  \vspace{-0.25in}
\end{wrapfigure}



% \begin{wrapfigure}{o}{0.35\textwidth}
%   \includegraphics[width=\linewidth]{figures/cos_sim_qa_hom.pdf}
%   \vspace{-0.25in}
%   \captionof{figure}{\small Avg. cos. sim. of gradients for QA model.}
%   \label{cos-sim-hom-qa}
%   \vspace{-0.15in}
% \end{wrapfigure}



==> cos_sim_plot_ner.tex <==

\begin{wrapfigure}{o}{0.27\textwidth}
  \includegraphics[width=\linewidth]{figures/cos_sim_ner.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Average cosine similarity between NER task gradients.}
  \label{cos-sim-ner}
  \vspace{-0.1in}
\end{wrapfigure}


==> cos_sim_plot_qa.tex <==
\begin{wrapfigure}{R}{0.27\textwidth}
\vspace{-0.1in}
  \includegraphics[width=\linewidth]{figures/cos_sim_qa.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Avg. cos. sim. between QA task gradients.}
  \label{cos-sim-qa}
  \smallskip\par
  \includegraphics[width=\linewidth]{figures/cos_sim_ner.pdf}
  \vspace{-0.3in}
  \captionof{figure}{\small Avg. cos. sim. between NER task gradients.}
  \label{cos-sim-ner}
  \vspace{-0.1in}
\end{wrapfigure}


% \begin{wrapfigure}{o}{0.27\textwidth}
% \vspace{-0.2in}
%   \includegraphics[width=\linewidth]{figures/cos_sim_qa.pdf}
%   \vspace{-0.3in}
%   \captionof{figure}{\small Average cosine similarity between QA task gradients.}
%   \label{cos-sim-qa}
%   \vspace{-0.1in}
% \end{wrapfigure}

==> lr_cos_plot.tex <==
\begin{wrapfigure}{R}{0.27\textwidth}
\vspace{-0.2in}
  \includegraphics[width=\linewidth]{figures/lr_cos_em.pdf}
  \vspace{-0.25in}
  \captionof{figure}{\small Plot of cos. sim. of QA task gradients and EM as a function of LR.}
  \label{lr-cos-em}
  \vspace{-0.15in}
\end{wrapfigure}

